Simulation of Vision-based Tactile Sensors using Physics based Rendering

Tactile sensing has seen a rapid adoption with the advent of vision-based tactile sensors. Vision-based tactile sensors provide high resolution, compact and inexpensive data to perform precise in-hand manipulation and human-robot interaction. However, the simulation of tactile sensors is still a challenge. In this paper, we built the first fully general optical tactile simulation system for a GelSight sensor using physics-based rendering techniques. We propose physically accurate light models and show in-depth analysis of individual components of our simulation pipeline. Our system outperforms previous simulation techniques qualitatively and quantitative on image similarity metrics. Our code and experimental data is open-sourced at https://labs.ri.cmu.edu/robotouch/tactile-optical-simulation/

==> comments.tex <==
wenzhen{\sout{The introduction need to be re-structured. A simple structure of introduction: \\
The big problem you are contributing to, why it's important -> \\
The small problem you are contributing to, why it's important -> \\}
The exact problem you try to solve-> \\
What's the must-know knowledge of this exact problem, and \sout{what's the current research status, what's their disadvantage and what's the challenge}-> \\
\sout{How did you approach the problem, and what's the result; why is your method a big contribution} ->\\
\sout{How is this project going to influence the big research field} and help the society
}

\wenzhen{You should also work on the language expression. Your audience are researchers in the general robotic area, so that they don't have knowledge on everything you mentioned here. Make sure everything in introduction is properly explained. And when you make a claim, and it's not some common knowledge, you need to explain it. }

\wenzhen{Since these sensors are the focus of your work and the object you are trying to model, you should give a brief overview about how they work}

\wenzhen{Somewhere you need to introduce the GelSight sensor: it's working principle, the design, and the algorithm/modeling used in the past. You can also talk about why it's an important sensor that it's valuable to simulate. Your audience might not know Gelsight (well), and they need some knowledge about what the sensor is like.}

\wenzhen{I think a better perspective to introduce the problem is like "Robot simulation is widely used (not only for machine learning), and important. But a major challenge for the current simulation environments is the lack of proper simulation for tactile sensing. This lead to the problem of XX, XX, XX... So we aim at building a good simulation tool for tactile sensors. Specifically we will work with this sensor, why .... "}

==> extra_text.tex <==
The modern machine learning techniques has led to tremendous progress in development of algorithms which can process rich sensory data and reason over long time horizons. However, in robotic manipulation the benefits of those algorithms have only been applied to visual stream. However, for dexterous human level manipulation estimating contacts\cite{calandra2017feeling} and associated properties like force, normals, location and shape are critical.

==> info.tex <==













\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

\section{}
Appendix two text goes here.



\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}



\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}


\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}






==> light_models.tex <==
We consider 3 light models to simulate LEDs, namely spotlight, IES light and directionally-varying area light(DVArea light). Figure \ref{comlightmodels} shows all the considered light models with the LEDs light used in our sensor. 


\begin{figure}[h]
\centering
  \includegraphics[width=\columnwidth,trim={0 0.2cm 0 0},clip]{pngs/lightcompare.png}
\caption{The comparison of the real LED photos and different light models. In the simulation setting, we view the lights directly from a front camera against a black wall, and placed extra hemispherical lenses on the lights for visualization purposes.}
\label{comlightmodels}
\end{figure}




\textit{Spot Light} is a point light source, which emits light rays directed in a cone. It has 2 parameters, namely the \textit{cutoff angle} and the \textit{beam width}. The cutoff angle is the angle of cone of light rays and beam width is the angle after which the light intensity falls off linearly from maximum value to zero.

\textit{IES light} is another point light source in which light intensity is given as a function of polar angles $\theta$ and $\phi$ of the emitted light ray. IES data is common data source given by the LED manufacturers(OSRAM in our case) in the form of 2D matrix of light intensity sampled at discrete known angle values. 

\textit{Directionally-varying area light} is the modified area light source, in which the outgoing light intensity is a functional of polar angles, similar to IES light. The directional attenuation is applied to each sampled point on the area light. The attenuation factor could be defined using a 2D matrix, like IES data matrix. 

For the point light model, we use 8-point light sources in a group; for the area light model, we use one source that is in the shape of the real LED line up. All the light sources show good match with the real light source as can be seen in Figure \ref{comlightmodels}. Different light models offer varying design choices, for example, IES lights are best when the manufacturer gives IES data; directionally-varying area light is fast to render and gives soft shadows; spot light is fastest to render and has easily tunable parameters. In this paper, we chose spot light model for our sensor simulation due to their high simulation speed and similar accuracy as compared to other light models.


==> macro.tex <==
% \usepackage[disable]{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{ulem}

\usepackage[numbers, square]{natbib}

\newcommand{\wenzhen}[1]{\todo[inline,color=red!40]{Wenzhen: #1}}
\newcommand{\arpit}[1]{\todo[inline,color=blue!20]{Arpit: #1}}

